On Algorithmic Decision Procedures in Emergency Response Systems in Smart and Connected Communities

Emergency Response Management (ERM) is a critical problem faced by communities across the globe. Despite this, it is common for ERM systems to follow myopic decision policies in the real world. Principled approaches to aid ERM decision-making under uncertainty have been explored but have failed to be accepted into real systems. We identify a key issue impeding their adoption --- algorithmic approaches to emergency response focus on reactive, post-incident dispatching actions, i.e. optimally dispatching a responder \textit{after} incidents occur. However, the critical nature of emergency response dictates that when an incident occurs, first responders always dispatch the closest available responder to the incident. We argue that the crucial period of planning for ERM systems is not post-incident, but between incidents. This is not a trivial planning problem --- a major challenge with dynamically balancing the spatial distribution of responders is the complexity of the problem. An orthogonal problem in ERM systems is planning under limited communication, which is particularly important in disaster scenarios that affect communication networks. We address both problems by proposing two partially decentralized multi-agent planning algorithms that utilize heuristics and exploit the structure of the dispatch problem. We evaluate our proposed approach using real-world data, and find that in several contexts, dynamic re-balancing the spatial distribution of emergency responders reduces both the average response time as well as its variance.

==> background.tex <==
\section{Related Work}



==> conclusion.tex <==
Principled approaches to Emergency Response Management (ERM) decision making have been explored, but have failed to be implemented into real systems. We have identified that a key issue with these approaches is that they focus on post-incident decision making. We argue that due to fairness constraints, planning should occur between incidents. We define a decision theoretic model for such planning, and implement a heuristic search using queuing theory as well as a multi-agent MCTS based planner. We find that these approaches maintain system fairness while decreasing the average response time to incidents. 

While the focus of this work is in the ERM domain, there are important takeaways for general agent-based systems: (1) Planning performance is dependent on the quality of the underlying event prediction models. (2) It is imperative to understand the needs and constraints for a target domain when designing a planning approach for it to be accepted in practice. (3) The computational capacity of ``agents'' has evolved in recent decades, and should be used to create decentralized planning approaches. Given these takeaways, we will explore the applicability of this framework to other domains where planning occurs over a spatial-temporally evolving process.

==> environment.tex <==
% \section{Environment}
% We will explore two possible representations for the underlying geographic area. In previous work, we used a grid based approach: the area is divided into 1x1 mile grid cells, and all the environmental state, incident predictions, and actions take place at the grid cell level. Incident models are learned for each cell, and responders respond to incidents by traveling to the cell the incident has occurred in. This approach works well for urban areas, as individual streets are too dense and incidents on individual streets are too rare to fit a model appropriately. 

% For interstates and more rural areas, we will be exploring a graph based approach, treating sections of the roads as edges in a graph and varying incident arrival rates. This will allow for 

==> formulation.tex <==
% \section{Formulation}
% Our goal is to develop an approach for emergency responder placement and incident response in a dynamic, continuous-time, stochastic environment. 
% We begin
% with several assumptions on the problem structure and information
% provided a priori. First, we assume that we are given a spatial map
% broken up into a finite collection of grids G, and assume that we
% are given an exogenous spatio-temporal model of incident arrival
% in continuous time over this collection of grids . Second, we assume that for each spatial grid cell, the temporal distribution of incidents is homogeneous.
% % This assumption is merely a reflection of the granularity of the
% % spatial discretization: we can in principle always discretize space
% % finely enough so that this assumption approximately holds. 
% Our third assumption is that emergency responders are allowed to be housed in a set of fixed and exogenously specified collection of depots, i.e. there are a subset of grid cells that responders can wait in. Each depot has a fixed capacity of responders it can house at a time. \ad{can they remain parked somewhere?}

% We assume that when an incident happens, a free responder (if
% available) is dispatched to the site of the incident. Once dispatched,
% the time to service consists of two parts: 1) time taken to travel to
% the scene of the incident, and 2) time taken to attend to the incident.
% If no free responders are available, then the incident enters a waiting
% queue. \ad{is this priority queues or a FCFS: FCFS now, as we have no severity}
% % We can naturally accommodate incidents with different
% % priorities in this framework by using a priority queue. Finally, we
% % assume that the distribution of vehicles in depots is given; it can
% % be calculated using a number of methods in the literature (e.g., [9]).
% Responders are allowed to move to any depot, as long as that depot is under capacity. \ad{is this possible (policy wise)? We can clairify what a depot is (station, parking spot, etc.) vs a fire station; possibly use different term}

% \ad{explain with map-reduce}
% We refer to the entire spatio-temporal process of incident arrival
% as well as the status of all responders and depots as our world. We
% consider the evolution of this world in continuous time. The dynamics of the world are primarily governed by two events that provide
% the scope of decision-making : occurrence of traffic incidents and
% completion of servicing. These are events when responders need to
% be either sent back to a depots or re-directed to other incidents. We also consider that responders can re-distribute themselves at time steps other than when these events occur if enough time has elapsed since the last event; we refer to these as  \textcolor{red}{balancing events.}
% Observe that the effect of these actions is not instantaneous. For
% example, when an incident happens and the action of dispatching a
% responder is taken, the occurrence of the next state is dependent on
% the time taken by the concerned responder to travel to the site and
% attend to the incident. Therefore, given a snapshot of our world
% (which we refer to as a state in our decision making process), the
% next state depends not only on the given state and the action taken,
% but also on how time evolves between the states.
% We model the continuous-time spatio-temporal dynamic decision problem faced by emergency responders using the machinery
% of Semi-Markov Decision Problems. We next describe each of the elements of the SMDP as it captures the emergency responder problem, while also explaining the special structure of this problem which is used for both representing and solving
% it.

% \subsection{States}
% A state at time $t$ is represented by $s^t$ which consists of a tuple
% $\{I^t, R^t\}$, where $I^t$
% is a collection of grid indices that are waiting
% to be serviced, ordered according to the relative times of incident
% occurrence. $ R^t$ corresponds to information about the set of responders
% at time $t$ with $|R^t| = b ∀t$, where b the total number of responders.
% Each entry $r^t_j \in R^t$ is a set $\{p^t_j,d^t_j,c^t_j\}$, where $p^t_j$ is the position of responder $j$, $d^t_j$ is the destination that it is traveling to (which can be its current position, and $c^t_j$ is its
% current condition, all observed at the state of our world at time t. $c^t_j \in {0, 1} \forall j,t$, with $c^t_j= 0$ meaning that the responder is currently engaged in service and not available for dispatch and $c^t_j= 1$ meaning that it is free and available to be dispatched. Finally, the set
% of all states is denoted by $S$.

% \subsection{Actions}
% Actions in our world correspond to directing all the responders to a valid grid cell to either respond to an incident or wait. Valid locations include grids with pending incidents and any depot that will not be over capacity. The valid grids for a specific state $s^i$ are denoted $V(s^i)$. We denote the set of all actions by $A$, with an action $a^i \in A$ corresponding to a set of sub actions $a^i_{rj}$, in which responder $r$ is moved to valid loaction $j \in V(s^i)$. $A(s^i)$ is the set of actions available in state $s^i \in S$

% % . In addition, we impose a
% % constraint that whenever responders are available and an incident
% % occurs, we always immediately dispatch some responder. 
% % We now
% % make several important observations. First, due to the continuous time nature of our model where a single incident arrives at any point in time, in our model of the world, at most a single action in A is ever taken. 

% % is this true with the new action space? 
% %This is a result of two model features: 1) since routing
% % a responder to an incident necessarily effects a state transition, and
% % 2) since we always respond to incidents if responders are available,
% % whenever we have multiple available responders, it must be the
% % case that there is at most one new incident to respond to.

% \subsection{World Evolution}

% We first look at how our world evolves before describing transitions.
% In our model, states evolve between events that provide the scope
% of decision-making . We refer to these times as decision epochs
% and such states as decision making states. For convenience, we
% segregate the three types of events (occurrence of incidents, and
% completion of servicing, and balancing) and refer to states in which responders
% become free as completion-states $S_c$, states in which incidents
% occur as incident-states $S_a$, and states in which balancing occurs as $S_b$. We also observe that states can evolve
% between decision epochs, and every such change in state does not
% present a chance to make decisions (i.e., the corresponding A(s)
% is empty). As an example, responders going to a depot
% move through different grids, which updates the state variable R,
% but presents no scope for decision making in our process, unless an
% incident or balancing event occurs. We also make the assumption that no two events can occur simultaneously in
% our world. In case such a scenario arises, since the world evolves in
% continuous time, we can add an infinitesimally small time interval
% to segregate the two events and create two separate states.
% In order to segregate decision making states from other states, we
% divide the model of our world into two processes as in prior work
% [12]: an embedded MDP that is observed only at decision epochs,
% and a natural process that evolves as if it is observed continuously
% through time, but presents no relevant information to the decision
% maker, unless the world is at a decision epoch. Since the decision
% making process is essentially the natural process observed at special
% (decision making) instances, the two processes are always the same
% at decision epochs. This segregation helps us in two ways: first, it
% truncates the state space by only looking at states that are relevant
% from the perspective of decision-making, and more importantly,
% it lets us remain agnostic about how the natural process evolves,
% thereby letting us exploit well-established models for transitions
% between our decision epochs.



% \subsection{Transitions}

% Having described the evolution of our world, we now look at
% both the transition time between events, as well as the probability
% of observing a state, given the last state and action taken. We define
% the former first, denoting the time between two states $s_i$
% and $s_j$ by
% the random variable $t_{ij}$. We denote the time between incidents by the random variable $t_a$, the time to service an incident by $t_s$, and the time to a balance step as $t_b$
% %We model interarrival times between incidents by using survival-analysis, that
% % has been widely used to model time to events, and has recently
% % been used to forecast urban incidents [9, 10], making it a natural
% % candidate for our purposes. Survival analysis is a broad class of
% % methods that are used to model the distribution of time and risk for
% % events. We use the accelerated time effect (AFT) model in which covariates increase or decrease the expected time to next incident [8],
% % letting us directly model time, rather than risk. Formally, we model
% % the time t between successive incidents as f (t|w), where t follows
% % an exponential distribution, and w is a set of arbitrary features
% % that affect t. As in standard AFT models, we model the arrival rate
% % for the exponential distribution as a log-linear model in terms of
% % the features w. Thus, the probability distribution of time to next
% % incident t
% % a
% % in a given spatial grid is

% % ----

% % where log λ
% % a =
% % Í
% % wj ∈W θjwj and θ are the regression coefficients
% % learned from data. This form of the model is particularly useful
% % to us in simulating our world, the purpose of which we explain
% % in Section 5. As in prior work [9], we model service time t
% % s by an
% % exponential distribution

% % ------

% Our models of $t_a$, $t_s$, and $t_b$ are crucial as they induce
% memoryless arrival and service times which allow us to model the
% entire dynamic dispatch process as an SMDP with special structure. $t_a$ is modeled using an exponential survival regression. $t_s$ is modeled by sampling from a distribution of service times and the time to travel to the incident given by a routing service. $t_b$ is a piecewise probability function with $p=0$ if the elapsed time since the last decision $\delta t$ is less than a blancing parameter $\alpha$, and $p=1 \text{if} \delta t >= \alpha$. 
% % To understand the temporal transitions, we first explain how time
% % evolves between two states by considering the following scenarios.
% % First, consider a series of two events as shown in Fig. 1, where at
% % time t1, an incident happens at grid i (state s
% % t 1
% % ) and a vehicle is
% % dispatched from grid j, and at time t2, the vehicle finishes servicing
% % the incident (state s
% % t2
% % ). The time between these two states is dt1t2
% % v+
% % t
% % s
% % , where dt1t2
% % is the distance between the concerned grids at states
% % s
% % t1 and s
% % t2 and v is the (known) velocity of the responders. Now, let
% % us consider the scenario that an incident or completion of service
% % happens at time t3, resulting in a new state s
% % t3
% % , such thatt1 < t3 < t2.
% % The time between states s
% % t3 and s
% % t2 now depends on whether the
% % responder traveling to grid j had reached its destination or not. If it
% % had not, we can calculate the distance left for it to travel and hence
% % the time tt3t2
% % based on information available in s
% % t3
% % . In case it had
% % reached and started servicing, we can leverage memorylessness of
% % the service time distribution and reset the remaining service time,
% % thereby estimating tt3t2
% % . Next, suppose that an incident happens
% % at time t1 (state s
% % t1
% % ), and the next incident occurs at time t2 (state
% % s
% % t2
% % ). The transition between incidents can be modeled directly by
% % the survival model in Eq. 1. Now, imagine that a new event (service
% % completion, state s
% % t3
% % ) happens at time t3 such that t1 < t3 < t2,
% % as shown in Fig. 2. Observe that since incident arrivals are also
% % memoryless, the time to state s
% % t2
% % , as seen from state s
% % t3 can again
% % be reset.

% % To summarize: 

% Having considered the temporal evolution between states, we
% now consider the probability of observing a state at a decision epoch,
% given a particular state at the last decision epoch and the associated
% action. We denote the probability that the process moves from state $s_i$ (at a decision epoch) to state $s_j$ (in the next decision epoch) under
% action a by $p_{ij}(a)$, where states belong to the embedded MDP. Note
% that the probability of transition between these states cannot solely
% be modeled using the incident, service time, and balancing distributions $f(t_a)$, $f(t_s)$, and $f(t_b)$, as the natural process evolves between decision epochs. $p_{ij}(a)$ thus captures the transition probabilities for states between decision epochs while taking into account the implicit evolution of the natural process. \textcolor{red}{Should we state a model for this? We don't have one now; it is modeled implicitly by the MCTS process}

% \subsection{Rewards}
% Rewards in SMDP usually have two components: a lump sum instantaneous reward for taking actions, and a continuous time reward
% as the process evolves. Our system only involves the former, which
% we denote by $\rho(s, a)$, for taking action $a$ in state $s$. We define the reward as $r = -t_s$, where $t_s$ is the response time to an incident. We are trying to maximize our reward, so it is negative. 




% \section{Constraints}




% \section{Assumptions}


% \section{Goals}

% \section{Emergency Response Management Decision Support Framework}

% \ad{merge this with the next section.}
% To effectively make dispatch recommendations online, a framework of interconnected processes is required. We base our framework on one designed by Mukhopadhyay et. al. \cite{mukhopadhyay2019online}, which is shown in figure \ref{fig:systemOverview} and includes the following components: 

% \begin{figure}%[t]
% \centering
% \includegraphics[width=\columnwidth]{Img/systemModelUpdated.pdf}
% \caption{ERM Framework Overview. \textcolor{red}{AD: the section headings are not applicable to this paper.}}
% \label{fig:systemOverview}
% \end{figure}

% \begin{itemize}
%     \item A traffic routing model to model the roadway network to support routing requests (e.g. how long it will take a responder to reach an incident or other destination) by the decision process
%     \item A model of the environment and how it changes over time, which is used by the incident prediction model
%     \item A model using past incident and environmental features to model the spatio-temporal distribution of incidents
%     \item A decision process that makes dispatching recommendations based on the current state of the environment, locations of responders, and likely future incident distributions. 
% \end{itemize}

% In this work we assume that the first three components are available, and focus purely on the decision process. 

% \textcolor{green}{add in figure and brief description of previous work \textit{that is being used}}

==> relatedResearch.tex <==
\section{Related Research}

%\subsection{Incident Dispatch Approaches}

The most obvious, and arguably the most commonly used policy for incident response in the real-world, is to follow a \textit{greedy} dispatch strategy: send the nearest available (in space) responder to an incident, i.e. maximize the myopic reward. This can result in decisions that sacrifice large future gains for small immediate rewards\cite{mukhopadhyay2019online}). 

Another approach to decision making is to directly solve the system's SMDP defined in \ref{sec:model} using policy iteration \cite{mukhopadhyayAAMAS18}. This poses a problem - the transition functions are unknown, and difficult to model in closed-form. To alleviate this, the Simulate-and-Transform (\textit{SimTrans}) algorithm\cite{mukhopadhyayAAMAS18} uses canonical Policy Iteration with an added computation. In order to estimate values (utilities) of states, the algorithm simulates the entire system of incident occurrence and responder dispatch and keeps track of all states transitions and actions, and gradually builds statistically confident estimates of the transition probabilities. While \emph{SimTrans} finds a close approximation of the optimal policy (assuming that the estimates of the transition probabilities learned are close to the true probabilities), this process is extremely slow and unsuited to dynamic environments.

To better react to shifting environmental conditions, online decision process approaches such as Monte Carlo Tree Search (MCTS) have been explored \cite{mukhopadhyay2019online}. MCTS is a class of heuristic-based search algorithms to find the most promising actions for a given state of a decision-making problem. Given an arbitrary state, MCTS repeatedly simulates the system under consideration to build a search tree that keeps track of the actions taken and the rewards received. The search tree is built in a manner that balances exploration (trying new or sub-optimal actions) and exploitation (greedily exploring the best action). As the number of search iterations increases, the search converges to the optimal action. As an anytime algorithm, MCTS is particularly well suited to the dispatch domain since it is trivial to balance the trade-off between computational time and solution quality. Also, given generative models of different components of the world (incident arrival, responder movement), it is easy to simulate the various complex interactions between agents and the environment.  

\iffalse
\subsection{Decentralized Monte Carlo Tree Search}
\textcolor{red}{Please add related research here about decentralized MCTS}


\subsection{Multi-agent Reinforcement Learning}
Problems similar to decentralized agent planning problem described in this paper have been studied in the context of developing multi-agent reinforcement learning approaches. Littman proposed a framework for multi-agent reinforcement learning that models the competition between two agents as a zero-sum Markov game~\cite{littman1994markov}.
To solve this game, the author introduced a Q-learning-like algorithm, called \emph{minimax-Q}, which is guaranteed to converge to optimal policies for both players.
However, the minimax-Q algorithm assumes that the game is zero sum (i.e., the player's rewards are exact opposites of each other) and every step of the training involves exhaustive searches over the action spaces, which limits the applicability of the algorithm. A number of follow up efforts have proposed more general solutions.

For example,
Hu and Wellman extended Littman's framework to general-sum stochastic games~\cite{hu1998multiagent}.
They propose an algorithm that is based on each agent learning two action-value functions (one for itself and one for its opponent), which is guaranteed to converge to a Nash equilibrium under certain conditions.
To relax some of these conditions, Littman introduced \emph{Friend-or-Foe Q-learning}, in which each agent is told to treat each other agent either as a ``friend'' or as a ``foe''~\cite{littman2001friend}. Later, Hu and Wellman proposed the \emph{NashQ algorithm}, which generalizes single-agent Q-learning to stochastic games with many agents by using an equilibrium operator instead of expected utility maximization~\cite{hu2003nash}.

Suttle et al.\ consider networked agents that communicate with their neighbors according to a time-varying graph, and collaboratively
evaluate and improve a target policy while following a distinct behavior policy~\cite{suttle2019multi}. However, this communication overhead is not suitable in our problem as it will not work if there are communication failures. 

Further, while the above approaches have the advantage of providing certain convergence guarantees, they assume that action-value functions are represented exactly, which is infeasible for scenarios with large action or state spaces, like in the problem described in this paper.
Deep multi-agent reinforcement-learning provides a more scalable approach by representing action-value functions using deep neural networks and may be an approach that we will revisit in future.
\fi
